Error-preserving Automatic Speech Recognition of Young English Learners' Language

One of the central skills that language learners need to practice is speaking the language. Currently, students in school do not get enough speaking opportunities and lack conversational practice. Recent advances in speech technology and natural language processing allow for the creation of novel tools to practice their speaking skills. In this work, we tackle the first component of such a pipeline, namely, the automated speech recognition module (ASR), which faces a number of challenges: first, state-of-the-art ASR models are often trained on adult read-aloud data by native speakers and do not transfer well to young language learners' speech. Second, most ASR systems contain a powerful language model, which smooths out errors made by the speakers. To give corrective feedback, which is a crucial part of language learning, the ASR systems in our setting need to preserve the errors made by the language learners. In this work, we build an ASR system that satisfies these requirements: it works on spontaneous speech by young language learners and preserves their errors. For this, we collected a corpus containing around 85 hours of English audio spoken by learners in Switzerland from grades 4 to 6 on different language learning tasks, which we used to train an ASR model. Our experiments show that our model benefits from direct fine-tuning on children's voices and has a much higher error preservation rate than other models.

==> tables/annotations.tex <==
\begin{table}[htbp]
    \scriptsize
    \centering
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{p{0.2\testcolwidth}p{0.4\testcolwidth}p{0.4\testcolwidth}}
        \toprule
        Convention & Description & Example\\
        \midrule
        German Words & Marked with @g. & He plays on the Wiese@g \\
        Best Guess & @? used for uncertain transcriptions. & It’s yellow and have@? a nice face. \\
        Errors & Marked with @!.  &  He play@! soccer. \\
        Missing Words & Indicated by @! in the correct place. & What @! you doing? \\
        Repetitions & Marked with a dash. & He’s - he's really tall. \\
        Reformulations & Marked with double dashes. & He’s -- he doesn’t like school. \\
        Long Pauses & Denoted with ellipses.  &  (…) \\
        \bottomrule
    \end{tabular}
    \caption{Transcription Symbols and Their Application in Annotating Non-Standard Speech}
    \label{tab:annotations}
\end{table}


==> tables/chall_xlsr_whisper_confusions.tex <==
 \begin{tabular}{|l|l|l|l|l|}
 \hline
  \textsc{Target}  & \textsc{Prediction} & \textsc{{Chall-300M}} & \textsc{Whisper-Large}  & \textsc{XLSR-1B} \\
    \hline
de@! & the & 331/350 & 312/359 & \textbf{ 276 }/343 \\
\hline
a@! & \_ & \textbf{ 89 }/779 & 257/787 & 270/778 \\
\hline
a@! & an & \textbf{ 20 }/779 & 313/787 & 200/778 \\
\hline
have@! & has & \textbf{ 12 }/795 & 182/789 & 41/783 \\
\hline
have@! & \_ & \textbf{ 27 }/795 & 101/789 & 101/783 \\
\hline
you@! & your & 54/221 & 68/222 & \textbf{ 22 }/223 \\
\hline
it's@! & it & \textbf{ 27 }/400 & 47/405 & 54/398 \\
\hline
it's@! & \_ & \textbf{ 17 }/400 & 48/405 & 58/398 \\
\hline
is@! & \_ & \textbf{ 19 }/377 & 48/384 & 51/376 \\
\hline
it's@! & is & \textbf{ 22 }/400 & 54/405 & 41/398 \\
\hline
are@! & \_ & \textbf{ 22 }/307 & 50/308 & 43/299 \\
\hline
dis@! & this & 41/48 & 39/47 & \textbf{ 33 }/46 \\
\hline
it@! & \_ & \textbf{ 16 }/171 & 57/183 & 34/176 \\
\hline
he@! & \_ & \textbf{ 24 }/137 & 34/134 & 47/132 \\
\hline
de@! & \_ & \textbf{ 10 }/350 & 44/359 & 49/343 \\
\hline
the@! & \_ & \textbf{ 9 }/195 & 49/204 & 37/202 \\
\hline
in@! & \_ & \textbf{ 8 }/291 & 38/300 & 31/290 \\
\hline
you@! & \_ & \textbf{ 17 }/221 & 25/222 & 26/223 \\
\hline
i@! & \_ & \textbf{ 13 }/98 & 25/101 & 30/102 \\
\hline
on@! & \_ & \textbf{ 5 }/264 & 34/263 & 27/257 \\
\hline
\end{tabular}

==> tables/chall_xlsr_whisper_correct.tex <==
 \begin{tabular}{|l|l|l|l|l|}
 \hline
  \textsc{Target}  & \textsc{Prediction} & \textsc{{Chall-300M}} & \textsc{Whisper-Large}  & \textsc{XLSR-1B} \\
    \hline
have@! & have & \textbf{ 696 }/795 & 463/789 & 547/783 \\
\hline
a@! & a & \textbf{ 626 }/779 & 169/787 & 253/778 \\
\hline
is@! & is & \textbf{ 298 }/377 & 256/384 & 289/376 \\
\hline
in@! & in & \textbf{ 261 }/291 & 232/300 & 234/290 \\
\hline
it's@! & it's & \textbf{ 281 }/400 & 230/405 & 192/398 \\
\hline
are@! & are & \textbf{ 227 }/307 & 212/308 & 209/299 \\
\hline
on@! & on & \textbf{ 242 }/264 & 197/263 & 203/257 \\
\hline
of@! & of & \textbf{ 177 }/192 & 134/190 & 162/191 \\
\hline
the@! & the & \textbf{ 159 }/195 & 129/204 & 137/202 \\
\hline
you@! & you & 134/221 & 122/222 & \textbf{ 164 }/223 \\
\hline
she@! & she & \textbf{ 137 }/158 & 112/157 & 120/155 \\
\hline
it@! & it & \textbf{ 132 }/171 & 106/183 & 116/176 \\
\hline
has@! & has & \textbf{ 113 }/137 & 107/138 & 106/137 \\
\hline
make@! & make & \textbf{ 115 }/121 & 91/122 & 97/120 \\
\hline
do@! & do & \textbf{ 105 }/128 & 96/129 & 95/127 \\
\hline
much@! & much & \textbf{ 97 }/99 & 96/100 & 95/99 \\
\hline
he@! & he & \textbf{ 93 }/137 & 84/134 & 74/132 \\
\hline
not@! & not & \textbf{ 89 }/100 & 78/104 & 80/103 \\
\hline
at@! & at & \textbf{ 90 }/111 & 71/116 & 85/112 \\
\hline
don't@! & don't & \textbf{ 85 }/96 & 76/92 & 77/95 \\
\hline
\end{tabular}

==> tables/chall_xlsr_whisper_correct__all_data.tex <==

 \begin{tabular}{|l|l|l|l|l|}
 \hline
  \textsc{Target}  & \textsc{Prediction} & \textsc{{Chall-300M}} & \textsc{Whisper-Large}  & \textsc{XLSR-1B} \\
    \hline


    \end{tabular}
